Investigating Deep Learning Benchmarks for Electrocardiography Signal Processing

In recent years, deep learning has witnessed its blossom in the field of Electrocardiography (ECG) processing, outperforming traditional signal processing methods in various tasks, for example, classification, QRS detection, wave delineation. Although many neural architectures have been proposed in the literature, there is a lack of systematic studies and open-source libraries for ECG deep learning. In this paper, we propose a deep learning framework, named \texttt{torch\_ecg}, which gathers a large number of neural networks, both from literature and novel, for various ECG processing tasks. It establishes a convenient and modular way for automatic building and flexible scaling of the networks, as well as a neat and uniform way of organizing the preprocessing procedures and augmentation techniques for preparing the input data for the models. Besides, \texttt{torch\_ecg} provides benchmark studies using the latest databases, illustrating the principles and pipelines for solving ECG processing tasks and reproducing results from the literature. \texttt{torch\_ecg} offers the ECG research community a powerful tool meeting the growing demand for the application of deep learning techniques.

==> main.tex <==
% use the following to switch among formats

% \input{main_jmlr}

\input{main_ieee_tran}

% \input{main_aims_mbe}
% \input{main_springer_lncs}
% \input{main_ws_jmmb}

% \input{review_revision/response_letter_1}

% \input{poster/baposter}


==> playground.tex <==

\begin{figure}
\centering
\begin{subfigure}[b]{.4\textwidth}
\centering
\begin{tikzpicture}[x=2.9cm, y=1.5cm, >=stealth, transform shape, scale=.9]

\foreach \m/\l [count=\y] in {1,...,5}
  \node [every neuron/.try, neuron \m/.try] (input-\m) at (0,3.5-\y) {$x_{\m}$};
  \node [neuron missing/.try] (input-missing) at (0,3.5-6) {};
  \node [every neuron/.try] (input-6) at (0,3.5-7) {$x_n$};

\foreach \h [count=\y] in {1,...,3}
  \node [every neuron/.try] (hidden-\h) at (2,3.2-\y*1.25) {$t_{\h}$};
  \node [neuron missing/.try] (hidden-missing) at (2,3.2-4*1.25) {};
  \node [every neuron/.try] (hidden-4) at (2,3.2-5*1.25) {$t_p$};

\foreach \i in {1,...,6}
  \foreach \j in {1,...,4}
    \draw [->] (input-\i) -- (hidden-\j);

\end{tikzpicture}
\caption{full connection}
\label{fig:full_con_nn}
\end{subfigure}\hfill
\begin{subfigure}[b]{.4\textwidth}
\centering
\begin{tikzpicture}[x=2.9cm, y=1.5cm, >=stealth, transform shape, scale=.9]

\foreach \m/\l [count=\y] in {1,...,5}
  \node [every neuron/.try, neuron \m/.try] (input-\m) at (0,3.5-\y) {$x_{\m}$};
  \node [neuron missing/.try] (input-missing) at (0,3.5-6) {};
  \node [every neuron/.try] (input-6) at (0,3.5-7) {$x_n$};

\foreach \h [count=\y] in {1,...,3}
  \node [every neuron/.try] (hidden-\h) at (2,3.2-\y*1.25) {$t_{\h}$};
  \node [neuron missing/.try] (hidden-missing) at (2,3.2-4*1.25) {};
  \node [every neuron/.try] (hidden-4) at (2,3.2-5*1.25) {$t_p$};

\foreach \i in {1,...,3}
    \draw [->] (input-\i) -- (hidden-1);
\foreach \i in {2,...,4}
    \draw [->] (input-\i) -- (hidden-2);
\foreach \i in {3,...,5}
    \draw [->] (input-\i) -- (hidden-3);
\draw [->] (input-6) -- (hidden-4);

\end{tikzpicture}
\caption{local connection}
\label{fig:local_con_nn}
\end{subfigure}
\caption{nn plot example}
\label{fig:nn}
\end{figure}

